Collective Intelligence for 2D Push Manipulations with Mobile Robots

While natural systems often present collective intelligence that allows them to self-organize and adapt to changes, the equivalent is missing in most artificial systems. We explore the possibility of such a system in the context of cooperative 2D push manipulations using mobile robots. Although conventional works demonstrate potential solutions for the problem in restricted settings, they have computational and learning difficulties. More importantly, these systems do not possess the ability to adapt when facing environmental changes. In this work, we show that by distilling a planner derived from a differentiable soft-body physics simulator into an attention-based neural network, our multi-robot push manipulation system achieves better performance than baselines. In addition, our system also generalizes to configurations not seen during training and is able to adapt toward task completions when external turbulence and environmental changes are applied. Supplementary videos can be found on our project website: https://sites.google.com/view/ciom/home

==> sections/03_background.tex <==
% \section{Problem Statement}

% We assume the multi robots are required to collectively push and manipulate a rope to a specified goal pose in an environment where the visual data from a camera of global view is available. From the global view, the rope state and the robots coordinates are obtained. Combining them and the goal state pre-defined, we design the observation space. In general, trajectories optimization are solved with sampling-based, reinforcement learning (RL). As for planner, multi-task RL is used.
% We employ incremental Intersection over Union (IoU) as our successful metric, defined as:
% \begin{displaymath}
% {incremental IoU} = \dfrac{{IoU({S}_{t}, {S}_{g})} - {IoU({S}_{0}, {S}_{g})}}{1 - {IoU({S}_{0}, {S}_{g})}}
% \end{displaymath}
% % \begin{displaymath}
% where IoU evaluate the how two point clouds have intersection.








% {IoU}_{({S}_{1}, {S}_{2})} = \dfrac{\sum_{ijk}\overline{S}_{1}\cdot\overline{S}_{2}}{\sum_{ijk}\overline{S}_{1} + \overline{S}_{2} - \overline{S}_{1}\cdot\overline{S}_{2}}
% \end{displaymath}
% \begin{displaymath}
% {S} = \dfrac{{S}}{{max}_{ijk}{S}^{ijk}}
% \end{displaymath}
% where ${S}^{xyz}$ stores how many materials are located in the grid point (x, y, z). 



% We assume the robots are required to collectively push and manipulate a deformable object to a specified goal pose in an environment where both visual data from a camera of global view and proprioceptive data are available. We formulate our rope manipulation task with multi robots into a Markov Decision Process (MDP) with state space ${S}$, action space ${A}$, observation space $\Omega$, deterministic transition dynamics $\mathcal{T}:{S}\times{A}\rightarrow{S}$ and mapping from states to observations ${O}:{S}\rightarrow\Omega$. In our simulation, our policy takes the ground-truth state information ${s}$, which includes the ground-truth point cloud of the rope, the ground-truth of the pose of the robots ${X}^{t}\in{SE(3)}$, and ground-truth point cloud of the target rope . We employ incremental IoU as our successful metric.

==> src/network.tex <==
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=\linewidth]{src/imgs/network.png}
    \caption{attention network.}
    \label{fig:network}
    \end{center}
\end{figure}

==> src/real2sim2real.tex <==
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.50\textwidth]{src/imgs/real2sim2real.png}
    \caption{realdemo}
    \label{fig:real2sim2real}
    \end{center}
\end{figure}

==> src/system.tex <==
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=\linewidth]{src/imgs/system.png}
    \caption{system setup overview.}
    \label{fig:system}
    \end{center}
\end{figure}
